Interconnected Kingdoms: Comparing 'A Song of Ice and Fire' Adaptations Across Media Using Complex Networks

In this article, we propose and apply a method to compare adaptations of the same story across different media. We tackle this task by modelling such adaptations through character networks. We compare them by leveraging two concepts at the core of storytelling: the characters involved, and the dynamics of the story. We propose several methods to match characters between media and compare their position in the networks; and perform narrative matching, i.e. match the sequences of narrative units that constitute the plots. We apply these methods to the novel series \textit{A Song of Ice and Fire}, by G.R.R. Martin, and its comics and TV show adaptations. Our results show that interactions between characters are not sufficient to properly match individual characters between adaptations, but that using some additional information such as character affiliation or gender significantly improves the performance. On the contrary, character interactions convey enough information to perform narrative matching, and allow us to detect the divergence between the original novels and its TV show adaptation.

==> tables/narr_match/comics-novels/perf_structural_blocks_smith-waterman.tex <==
\begin{tabular}{lrrrr}
\toprule
Jaccard index & \multicolumn{2}{c}{nodes} & \multicolumn{2}{c}{edges} \\
weighted & no & yes & no & yes \\
character filtering &  &  &  &  \\
\midrule
Named & 71.81 & 70.95 & 71.52 & 71.38 \\
Common & 70.23 & \bfseries 72.30 & 71.14 & 71.57 \\
Top-20 & 60.93 & 63.33 & 49.35 & 59.93 \\
\bottomrule
\end{tabular}

==> tables/narr_match/comics-novels/perf_structural_blocks_treshold.tex <==
\begin{tabular}{lrrrr}
\toprule
Jaccard index & \multicolumn{2}{c}{nodes} & \multicolumn{2}{c}{edges} \\
weighted & no & yes & no & yes \\
character filtering &  &  &  &  \\
\midrule
Named & 16.42 & 14.80 & 24.80 & 25.66 \\
Common & 19.84 & 23.82 & 27.95 & \bfseries 33.23 \\
Top-20 & 8.24 & 7.77 & 11.33 & 14.04 \\
\bottomrule
\end{tabular}

==> tables/narr_match/comics-novels/perf_structural_comics-novels-c2c.tex <==
\begin{tabular}{lllrrr}
\toprule
Representation & Measure & Alignment & \multicolumn{3}{c}{\itshape Novels vs. Comics} \\
 &  &  & \ttfamily named & \ttfamily common & \ttfamily top-20 \\
\midrule
\multirow[c]{4}{*}{Edges} & \multirow[c]{2}{*}{Jaccard} & Smith--Waterman & 69.62 & 69.62 & 39.42 \\
 &  & Thresholding & 27.94 & 31.68 & 11.85 \\
\cmidrule{2-6}
 & \multirow[c]{2}{*}{Ru\v{z}i\v{c}ka} & Thresholding & 28.60 & 38.52 & 14.95 \\
 & & Smith--Waterman & \bfseries 70.06 & 69.18 & 52.75 \\
\cmidrule{1-6}
\multirow[c]{4}{*}{Vertices} & \multirow[c]{2}{*}{Jaccard} & Thresholding & 17.55 & 21.25 & 8.00 \\
& & Smith--Waterman & \bfseries 70.06 & 69.21 & 56.70 \\
\cmidrule{2-6}
 & \multirow[c]{2}{*}{Ru\v{z}i\v{c}ka} & Thresholding & 15.19 & 26.01 & 6.71 \\
& & Smith--Waterman & 69.84 & 69.84 & 58.68 \\
\bottomrule
\end{tabular}

==> tables/narr_match/tvshow-novels/perf_structural_blocks_smith-waterman.tex <==
\begin{tabular}{lrrrr}
\toprule
Jaccard index & \multicolumn{2}{c}{nodes} & \multicolumn{2}{c}{edges} \\
weighted & no & yes & no & yes \\
character filtering &  &  &  &  \\
\midrule
Named & 31.78 & 34.46 & 33.17 & 31.33 \\
Common & 32.16 & \bfseries 35.09 & 31.58 & 34.38 \\
Top-20 & 30.69 & 25.91 & 22.54 & 24.33 \\
\bottomrule
\end{tabular}

==> tables/narr_match/tvshow-novels/perf_structural_blocks_threshold.tex <==
\begin{tabular}{lrrrr}
\toprule
Jaccard index & \multicolumn{2}{c}{nodes} & \multicolumn{2}{c}{edges} \\
weighted & no & yes & no & yes \\
character filtering &  &  &  &  \\
\midrule
Named & 15.32 & 15.62 & 17.79 & \bfseries 21.02 \\
Common & 12.54 & 17.63 & 17.00 & 18.72 \\
Top-20 & 6.42 & 6.55 & 6.79 & 7.74 \\
\bottomrule
\end{tabular}
